R-MBO: A Multi-surrogate Approach for Preference Incorporation in Multi-objective Bayesian Optimisation

Many real-world multi-objective optimisation problems rely on computationally expensive function evaluations. Multi-objective Bayesian optimisation (BO) can be used to alleviate the computation time to find an approximated set of Pareto optimal solutions. In many real-world problems, a decision-maker has some preferences on the objective functions. One approach to incorporate the preferences in multi-objective BO is to use a scalarising function and build a single surrogate model (mono-surrogate approach) on it. This approach has two major limitations. Firstly, the fitness landscape of the scalarising function and the objective functions may not be similar. Secondly, the approach assumes that the scalarising function distribution is Gaussian, and thus a closed-form expression of an acquisition function e.g., expected improvement can be used. We overcome these limitations by building independent surrogate models (multi-surrogate approach) on each objective function and show that the distribution of the scalarising function is not Gaussian. We approximate the distribution using Generalised value distribution. We present an a-priori multi-surrogate approach to incorporate the desirable objective function values (or reference point) as the preferences of a decision-maker in multi-objective BO. The results and comparison with the existing mono-surrogate approach on benchmark and real-world optimisation problems show the potential of the proposed approach.

==> BO.tex <==
This will cover the Gaussian processes and expected improvement



==> laplace_calculations.tex <==
\subsection*{Laplace approximation calculations for bi-objective optimisation}



Let us denote $mi = w_i(\mu_i - z_i^*)$ and $si = w_i \sigma_i$, where $\mu_i$, $\sigma_i$, $z_i^*$ and $w_i$ are the $i^{th}$ element of the posterior mean vector, the standard deviation vector, the desirable objective vector and the weight vector, respectively. The distribution of $g$ mentioned in Equation (\ref{eq:g_pdf2}) can also be written as:
{\fontsize{6}{10}\selectfont
% \begin{doublespace}
\begin{equation}
 p(g) = \frac{1}{4}\text{Erfc}\left[-\frac{g-\text{m1}}{\sqrt{2}\text{s1}}\right]\left(\frac{e^{-\frac{(g-\text{m1})^2}{2\text{s1}^2}}\sqrt{\frac{2}{\pi}}}{\text{s1}\text{Erfc}\left[-\frac{g-\text{m1}}{\sqrt{2}\text{s1}}\right]}+\frac{e^{-\frac{(g-\text{m2})^2}{2\text{s2}^2}}\sqrt{\frac{2}{\pi}}}{\text{s2}\text{Erfc}\left[-\frac{g-\text{m2}}{\sqrt{2}\text{s2}}\right]}\right)\text{Erfc}\left[-\frac{g-\text{m2}}{\sqrt{2} \text{s2}}\right] 
\end{equation}
}


The mode, $g_0$ can be calculated by taking the derivative of the $\log g$ i.e.\ $\frac{d \log g}{d g}$ =0:
\tiny{
\begin{dmath}
\frac{4 \text{s1}^2 \text{s2}^2+\sqrt{2 \pi } \left(-e^{\frac{(g-\text{m1})^2}{2 \text{s1}^2}} (g-\text{m2}) \text{s1}^3 \text{Erfc}\left[\frac{-g+\text{m1}}{\sqrt{2}
\text{s1}}\right]-e^{\frac{(g-\text{m2})^2}{2 \text{s2}^2}} (g-\text{m1}) \text{s2}^3 \text{Erfc}\left[\frac{-g+\text{m2}}{\sqrt{2} \text{s2}}\right]\right)}{\sqrt{2
\pi } \text{s1}^2 \text{s2}^2 \left(e^{\frac{(g-\text{m1})^2}{2 \text{s1}^2}} \text{s1} \text{Erfc}\left[\frac{-g+\text{m1}}{\sqrt{2} \text{s1}}\right]+e^{\frac{(g-\text{m2})^2}{2
\text{s2}^2}} \text{s2} \text{Erfc}\left[\frac{-g+\text{m2}}{\sqrt{2} \text{s2}}\right]\right)} =0
\end{dmath}}

\normalsize{The equation does not have a closed form expression for estimating the mode. Therefore, the mode can be estimated by maximising a posteriori with an iterative method e.g.\ Newton's method.}

 


\normalsize{Once the mode is known, we can estimate the second derivative at the mode:}
% {\fontsize{4}{6}\selectfont
\tiny{
\begin{dmath}
    A = -\diff*[2]{\log g}{g}{g = g_0} = \left(-e^{\frac{(g-\text{m1})^2}{\text{s1}^2}} \pi  \text{s1}^5 \text{s2} \text{Erfc}\left[\frac{-g+\text{m1}}{\sqrt{2} \text{s1}}\right]^2+e^{\frac{(g-\text{m1})^2}{2
\text{s1}^2}} \text{Erfc}\left[\frac{-g+\text{m1}}{\sqrt{2} \text{s1}}\right] \left(\sqrt{2 \pi } \text{s1}^2 \text{s2} \left((g-\text{m2}) \text{s1}^2+3
(-g+\text{m1}) \text{s2}^2\right)+e^{\frac{(g-\text{m2})^2}{2 \text{s2}^2}} \pi  \left((g-\text{m2})^2 \text{s1}^4-\text{s1}^2 \left(2 (g-\text{m1})
(g-\text{m2})+\text{s1}^2\right) \text{s2}^2+(g-\text{m1}-\text{s1}) (g-\text{m1}+\text{s1}) \text{s2}^4\right) \text{Erfc}\left[\frac{-g+\text{m2}}{\sqrt{2}
\text{s2}}\right]\right)-\text{s1} \text{s2}^2 \left(8 \text{s1}^2 \text{s2}+e^{\frac{(g-\text{m2})^2}{2 \text{s2}^2}} \sqrt{2 \pi } \left(3 (g-\text{m2})
\text{s1}^2+(-g+\text{m1}) \text{s2}^2\right) \text{Erfc}\left[\frac{-g+\text{m2}}{\sqrt{2} \text{s2}}\right]+e^{\frac{(g-\text{m2})^2}{\text{s2}^2}}
\pi  \text{s2}^3 \text{Erfc}\left[\frac{-g+\text{m2}}{\sqrt{2} \text{s2}}\right]^2\right)\right)/\left(\pi  \text{s1}^3 \text{s2}^3 \left(e^{\frac{(g-\text{m1})^2}{2
\text{s1}^2}} \text{s1} \text{Erfc}\left[\frac{-g+\text{m1}}{\sqrt{2} \text{s1}}\right]+e^{\frac{(g-\text{m2})^2}{2 \text{s2}^2}} \text{s2} \text{Erfc}\left[\frac{-g+\text{m2}}{\sqrt{2}
\text{s2}}\right]\right)^2\right)
\end{dmath}
}

\normalsize{After estimating the mode and the second derivative at the mode, the distribution of $g$ can be written as:
\begin{align*}
    g \sim \mathcal{N}(g_0, A^{-1}),
\end{align*}}
where $g_0$ is the mean and $A^{-1}$ is the variance. These calculations allow us to use the closed form expression of acquisition functions e.g.\ expected improvement and probability of improvement. 

